Illusion: Safeguarding Topology Confidentiality in LLM Multi-Agent Systems via Behavior-Preserving Obfuscation

The communication topology of Large Language Model Multi-Agent Systems (LLM-MASs) governs how information propagates among agents and encodes critical domain knowledge and expert workflow design. It is valuable intellectual property and plays a decisive role in system utility and safety, yet remains vulnerable to inference attacks that stealthily reconstruct it from agent outputs. Existing defenses detect or mitigate such attacks but do not proactively conceal the topology itself. We propose \textit{Illusion}, a proactive topology obfuscation defense for LLM-MAS. \textit{Illusion} injects fake edges and fake messages to present attackers with a deceptive topology, while selecting low-impact candidates that preserve output-distribution equivalence and task-accuracy non-inferiority. The resulting fake edges are designed to be indistinguishable from genuine messages under black-box observation. Extensive experiments show that \textit{Illusion} reduces edge-level F1 from over 0.87 to 0.62 and graph similarity from over 0.94 to 0.71. It also largely preserves output distributions and task performance, and its fake edges resist both similarity-based and LLM-judge filtering, even under adaptive pruning.

==> header.tex <==

\makeatletter

%% ---- 1. Packages ---------------------------------------------------
\PassOptionsToPackage{dvipsnames,table,xcdraw}{xcolor}
\usepackage{acronym}
\usepackage{xcolor}  
\usepackage{enumitem}
% colors
\usepackage{colortbl}        % \cellcolor, \rowcolor, \arrayrulecolor (even if xcolor was loaded without "table")
\usepackage{xspace}          % spacing after text macros
\usepackage{array}           % P column type, m{} columns
\usepackage{booktabs}        % \specialrule in the table helpers
\usepackage{forloop}         % Gantt-chart helpers
\usepackage{relsize}         % \smaller in \cc
\usepackage{graphicx}        % \scalebox, \includegraphics
\usepackage{pifont}          % \cmark, \xmark
\usepackage{tikz}
\usetikzlibrary{shapes,arrows.meta,positioning,fit,backgrounds,calc}
\usepackage{fontawesome5}    % icons: \faEdit, \faFlask, \faCloud, ...
\usepackage{tcolorbox}
\tcbuselibrary{skins,breakable}
\usepackage{amsmath}
%% ---- 2. Color palette ----------------------------------------------
%% Figure and box palette (inspired by crimson/gray/gold slide styles).
\providecolor{gcred}{HTML}{C8102E}        % crimson accent
\providecolor{gcgold}{HTML}{FFCD00}       % gold highlight
\providecolor{gcgolddark}{HTML}{8A6A00}   % gold that is readable as text
\providecolor{gcgray}{gray}{0.55}         % bracket/label gray (= black!45)
\providecolor{gcpanel}{gray}{1}           % figure panel fill (white)
\providecolor{todocolor}{HTML}{C2410C}    % draft notes (burnt orange)
\providecolor{lightgreen}{RGB}{213,242,184} % Gantt "on" cells
%% Fallbacks for dvipsnames colors used by the author notes (if xcolor was loaded without dvipsnames).
\providecolor{ForestGreen}{cmyk}{0.91,0,0.88,0.12}
\providecolor{RubineRed}{cmyk}{0,1,0.13,0}


% \usepackage{hyperref}
% \hypersetup{
%  colorlinks=true,      % false: boxed links; true: colored links
%  linkcolor=blue,       % color of internal links
%  citecolor=red,    % color of links to bibliography
%  filecolor=cyan,       % color of file links
%  urlcolor=magenta          % color of external links
% }


%% ---- 3. Draft notes and author notes -------------------------------
%% \todo{...}: a small "TODO" tag followed by the note in sans-serif.
%% Every note is written to the log, with a total at the end of the build.
%% \showtodosfalse hides the notes; the log count still reports them.
\ifdefined\ifshowtodos\else
  \newif\ifshowtodos \showtodostrue
\fi
\@ifundefined{c@todocount}{\newcounter{todocount}}{}
\DeclareRobustCommand{\todo}[1]{%
  \stepcounter{todocount}%
  \typeout{[TODO \thetodocount] \detokenize{#1}}%
  \ifshowtodos
    \unskip\hspace{0.3em}%
    \tikz[baseline=(todotag.base)]\node[fill=todocolor, rounded corners=1.5pt, inner sep=1.4pt,
      text=white, font=\sffamily\bfseries\scriptsize] (todotag) {\faEdit\,TODO};%
    \nobreak\hspace{0.25em}{\sffamily\small\color{todocolor}#1}%
  \fi}
\AtEndDocument{\typeout{==== \thetodocount\space TODO note(s) in this build ====}}

%% Inline author notes.
\providecommand{\hnote}[1]{{$\langle${\textcolor{ForestGreen}{Hao: {#1}}}$\rangle$}}
\providecommand{\jnote}[1]{{$\langle${\textcolor{RubineRed}{Jian: {#1}}}$\rangle$}}
\providecommand{\hao}[1]{{\textcolor{ForestGreen}{{#1}}}}
\@ifundefined{c@notesec}{\newcounter{notesec}[section]}{}
\providecommand{\thenoteee}{\thesection.\arabic{notesec}}
\providecommand{\xz}[1]{\refstepcounter{notesec}{\bf\textcolor{blue}{$\ll$XZ~\thenoteee: {\sf #1}$\gg$}}}
\providecommand{\xzh}[1]{\refstepcounter{notesec}{\bf\textcolor{red}{$\ll$XZ~\thenoteee: @Hao, {\sf #1}$\gg$}}}
\providecommand{\blue}[1]{\textcolor{blue}{#1}}
\providecommand{\red}[1]{\textcolor{red}{#1}}

%% ---- 4. Writing shortcuts and run-in headings ----------------------
\providecommand{\eg}{\textit{e.g.}}
\providecommand{\ie}{\textit{i.e.}}
\providecommand{\etc}{\textit{etc}}
\providecommand{\etal}{\textit{et al}.\xspace}
\providecommand{\bheading}[1]{{\vspace{2pt}\noindent{\textbf{#1}}}}  % bold run-in heading
\providecommand{\iheading}[1]{{\vspace{2pt}\noindent{\textit{#1}}}}  % italic run-in heading
\providecommand{\ind}{\hspace{6mm}}
\providecommand*{\TitleFont}{\usefont{\encodingdefault}{\rmdefault}{b}{n}\fontsize{15}{15}\selectfont}
\providecommand{\ignore}[1]{}
\providecommand{\cc}[1]{\mbox{\smaller[0.5]\texttt{#1}}}                             % small code
\providecommand{\bcc}[1]{\mbox{\smaller[0.5]\textcolor{blue!20!black}{\texttt{#1}}}} % small code, tinted
\providecommand{\tabref}[1]{\mbox{Table~\ref{#1}}}
\providecommand{\secrefs}[2]{\mbox{Sec.~\ref{#1}--\ref{#2}}\xspace}
\providecommand{\lstref}[1]{\mbox{Listing~\ref{#1}}}
\providecommand{\nalgref}[1]{\mbox{Alg.~\ref{#1}}}
\providecommand{\cmark}{\ding{51}}
\providecommand{\xmark}{\ding{55}}

%% ---- 5. Compact lists ----------------------------------------------
\@ifundefined{packeditemize}{%
  \newenvironment{packeditemize}{%
    \begin{list}{$\bullet$}{%
      \setlength{\itemsep}{0pt}\setlength{\labelwidth}{8pt}%
      \setlength{\leftmargin}{10pt}\setlength{\labelsep}{3pt}%
      \setlength{\listparindent}{\parindent}\setlength{\parsep}{1.5pt}%
      \setlength{\parskip}{1.5pt}\setlength{\topsep}{1.5pt}}}%
    {\end{list}}}{}
\@ifundefined{c@packednmbr}{\newcounter{packednmbr}}{}
\@ifundefined{packedenumerate}{%
  \newenvironment{packedenumerate}{%
    \begin{list}{\thepackednmbr.}{\usecounter{packednmbr}%
      \setlength{\itemsep}{0pt}\addtolength{\labelwidth}{4pt}%
      \setlength{\leftmargin}{12pt}\setlength{\listparindent}{\parindent}%
      \setlength{\parsep}{3pt}\setlength{\topsep}{3pt}}}%
    {\end{list}}}{}

%% ---- 6. Cross-reference names for \autoref -------------------------
%% \autoref{sec:x} -> "§2" (no space), \autoref{fig:x} -> "Fig. 1".
%% Applied at \begin{document} so that hyperref/babel defaults are overridden.
%% (\autoref itself comes from hyperref; without hyperref use \ref.)
\def\Snospace~{\S{}}
\AtBeginDocument{%
  \def\sectionautorefname{\Snospace}%
  \def\subsectionautorefname{\Snospace}%
  \def\subsubsectionautorefname{\Snospace}%
  \def\chapterautorefname{\Snospace}%
  \def\figureautorefname{Fig.}%
  \def\figurename{Fig.}}

%% ---- 7. Figures: icon helper and pgf layers ------------------------
%% \gcicon{icon}{label}: crimson icon on the left, label on the right
%% (used inside TikZ boxes). Widths can be changed via the two macros.
\providecommand{\gciconwidth}{0.66cm}
\providecommand{\gcicontextwidth}{1.94cm}
\providecommand{\gcicon}[2]{\begin{tabular}{@{}>{\centering\arraybackslash}m{\gciconwidth}@{\hspace{3pt}}%
    >{\raggedright\arraybackslash\hyphenpenalty=10000\exhyphenpenalty=10000}m{\gcicontextwidth}@{}}%
    {\color{gcred}\scalebox{0.8}{\LARGE #1}} & #2\end{tabular}}
%% Extra layer drawn behind TikZ's "background" layer (for panels behind groups).
%% Note: this sets the global pgf layer order.
\pgfdeclarelayer{backmost}
\pgfsetlayers{backmost,background,main}

%% ---- 8. Case-study boxes -------------------------------------------
%% \begin{casebox}{label}{title}{fill color}{title color} ... \end{casebox}
%% Rounded box, plain light fill, no border; breaks across pages.
\@ifundefined{casebox}{%
  \newtcolorbox{casebox}[4]{%
    enhanced, breakable, arc=6pt, frame hidden,
    colback=#3,
    left=6pt, right=6pt, top=3pt, bottom=3pt, boxsep=2pt,
    fontupper=\small, before skip=6pt, after skip=6pt,
    before upper={\textbf{(#1)}\ \textcolor{#4}{\textbf{#2}}\par\smallskip}}}{}
%% \caseitem{icon}{label}{text}: icon-led line with a hanging indent.
\providecommand{\caseitem}[3]{\par\noindent\hangindent=1.5em\hangafter=1%
  \makebox[1.5em][l]{\color{gcred}#1}\textbf{#2.}\ #3}

%% ---- 9. Tables -----------------------------------------------------
\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}   % centered fixed-width column
%% Gantt-chart helpers for timeline tables:
%%   \rpt[n]{x} repeats x n times; \on[n] adds n shaded cells; \off[n] adds n empty cells.
\@ifundefined{c@loopcntr}{\newcounter{loopcntr}}{}
\providecommand{\rpt}[2][1]{\forloop{loopcntr}{0}{\value{loopcntr}<#1}{#2}}
\providecommand{\on}[1][1]{\forloop{loopcntr}{0}{\value{loopcntr}<#1}{&\cellcolor{lightgreen}}}
\providecommand{\off}[1][1]{\forloop{loopcntr}{0}{\value{loopcntr}<#1}{&}}
%% Shaded single cells.
\providecommand{\SH}{\multicolumn{1}{>{\columncolor{darkgray}}l|}{}}
\providecommand{\SM}{\multicolumn{1}{>{\columncolor{gray}}l|}{}}
\providecommand{\SL}{\multicolumn{1}{>{\columncolor{lightgray}}l}{}}
%% Row colors and colored booktabs-style rules.
\colorlet{tableheadcolor}{gray!25}
\colorlet{tablerowcolor}{gray!10}
\colorlet{tablerowcolortwo}{gray!25}
\colorlet{tablerowcolorthree}{gray!40}
\providecommand{\headcol}{\rowcolor{tableheadcolor}}
\providecommand{\rowcol}{\rowcolor{tablerowcolor}}
\providecommand{\rowcoltwo}{\rowcolor{tablerowcolortwo}}
\providecommand{\rowcolthree}{\rowcolor{tablerowcolorthree}}
\providecommand{\topline}{\arrayrulecolor{black}\specialrule{0.1em}{\abovetopsep}{0pt}%
  \arrayrulecolor{tableheadcolor}\specialrule{\belowrulesep}{0pt}{0pt}\arrayrulecolor{black}}
\providecommand{\midline}{\arrayrulecolor{tableheadcolor}\specialrule{\aboverulesep}{0pt}{0pt}%
  \arrayrulecolor{black}\specialrule{\lightrulewidth}{0pt}{0pt}%
  \arrayrulecolor{white}\specialrule{\belowrulesep}{0pt}{0pt}\arrayrulecolor{black}}
\providecommand{\bottomline}{\arrayrulecolor{white}\specialrule{\aboverulesep}{0pt}{0pt}%
  \arrayrulecolor{black}\specialrule{\heavyrulewidth}{0pt}{\belowbottomsep}}

%% ---- 10. Units -----------------------------------------------------
\providecommand{\bytes}{\ensuremath{\mathrm{B}}\xspace}
\providecommand{\kbytes}{\ensuremath{\mathrm{KB}}\xspace}
\providecommand{\mbytes}{\ensuremath{\mathrm{MB}}\xspace}
\providecommand{\gbytes}{\ensuremath{\mathrm{GB}}\xspace}
\providecommand{\gbits}{\ensuremath{\mathrm{Gb}}\xspace}
\providecommand{\hertz}{\ensuremath{\mathrm{Hz}}\xspace}
\providecommand{\ghertz}{\ensuremath{\mathrm{GHz}}\xspace}
\providecommand{\secs}{\ensuremath{\mathrm{s}}\xspace}
\providecommand{\msecs}{\ensuremath{\mathrm{ms}}\xspace}
\providecommand{\usecs}{\ensuremath{\mathrm{\mu{}s}}\xspace}
\providecommand{\nsecs}{\ensuremath{\mathrm{ns}}\xspace}

%% ---- 11. Math shortcuts and theorem environments -------------------
\providecommand{\bbR}{\mathbb{R}}
\providecommand{\calN}{\mathcal{N}}
\providecommand{\calR}{\mathcal{R}}
\providecommand{\calV}{\mathcal{V}}
\providecommand{\w}{\textbf{w}}
\providecommand{\s}{\textbf{s}}
\providecommand{\g}{\textbf{g}}
\@ifundefined{theorem}{\newtheorem{theorem}{Theorem}[section]}{}
\@ifundefined{definition}{\newtheorem{definition}{Definition}}{}
\@ifundefined{lemma}{\newtheorem{lemma}{Lemma}}{}
\@ifundefined{example}{\newtheorem{example}{Example}}{}

\makeatother
\endinput


